PECon: Contrastive Pretraining to Enhance Feature Alignment between CT and EHR Data for Improved Pulmonary Embolism Diagnosis

Previous deep learning efforts have focused on improving the performance of Pulmonary Embolism(PE) diagnosis from Computed Tomography (CT) scans using Convolutional Neural Networks (CNN). However, the features from CT scans alone are not always sufficient for the diagnosis of PE. CT scans along with electronic heath records (EHR) can provide a better insight into the patients condition and can lead to more accurate PE diagnosis. In this paper, we propose Pulmonary Embolism Detection using Contrastive Learning (PECon), a supervised contrastive pretraining strategy that employs both the patients CT scans as well as the EHR data, aiming to enhance the alignment of feature representations between the two modalities and leverage information to improve the PE diagnosis. In order to achieve this, we make use of the class labels and pull the sample features of the same class together, while pushing away those of the other class. Results show that the proposed work outperforms the existing techniques and achieves state-of-the-art performance on the RadFusion dataset with an F1-score of 0.913, accuracy of 0.90 and an AUROC of 0.943. Furthermore, we also explore the explainability of our approach in comparison to other methods. Our code is publicly available at https://github.com/BioMedIA-MBZUAI/PECon.

==> Tables/results.tex <==
% \begin{table*}[]
% \label{tab:results}
% \caption{\centering Summary of results.}

%         \resizebox{1\linewidth}{!}{\begin{tabular}{l c c c c c c} 
%          & Optimal Threshold & Accuracy & F1-score & Specificity & Sensitivity & AUROC\\ % Amalgamating several columns into one cell is done using the \multicolumn command with the number of columns to amalgamacmate as the first argument and then the justification (l, r or c)
%         \midrule% Horizontal line spanning less than the full width of the table - you can add (r) or (l) just before the opening curly bracket to shorten the rule on the left or right side

%         1 HG & 57.44 & 67.85 & 65.57 & 60.44 \\ % 
%         \textbf{2 HG} & 58.12 & 69.67 &69.08 & 63.35  \\
%         3 HG & 57.91 & 70.30 & 69.81 & 64.59 \\
%         %% Content row 5
%         \midrule
%             \multicolumn{7}{c}{\textbf{\rule{0pt}{2pt}{Imaging-only models}}} \\
%         \midrule
%         Ghost bottleneck & 56.68 & 65.62 & 61.96 & 53.45& 57.99& 57.99\\ 
%         Shuffle bottleneck &  55.66 & 64.76 & 61.96  &  55.16& 57.99& 57.99\\ 
%         DiCE bottleneck & 56.65 & 68.27 & 66.85&  61.16& 57.99& 57.99 \\ 
%         \midrule
%             \multicolumn{7}{c}{\textbf{\rule{0pt}{2pt}{EHR-only models}}}\\
%         \midrule
%         Dilated bottleneck &  57.57   &    69.29    &69.17&    64.16& 57.99& 57.99\\ 
%         Dilated bottleneck & 57.88       & 69.34   & 68.11 &   62.50& 57.99& 57.99\\ 
%         Multidilated in HG & 57.54 &  69.43 & 68.69 &   63.99& 57.99& 57.99\\ 
%         Multidilated everywhere &  57.88&  69.29 & 68.72 &   63.90& 57.99& 57.99 \\ 
%         \midrule
%             \multicolumn{7}{c}{\textbf{\rule{0pt}{2pt}{Multi-modal fusion models}}} \\\midrule
%         Weighted $L_{percept}$ & 56.62 & 66.58 & 62.79 & 57.99& 57.99& 57.99 \\
%         Low channels & 57.74 & 68.65 & 67.67 & 62.56 &63.39 &63.39 \\ % Content row 2
%         Fully separable & 57.61 & 69.31& 63.39 &63.39 & 68.54 & 62.91\\ % Content row 3
%         Separable $ResConcat$ &  \textbf{58.36} & \textbf{69.40} & \textbf{68.45} & \textbf{63.64}& 63.39 &63.39 \\
%         Separable ${ResConcat}$ & 56.72 & 66.00 & 63.39 & 63.39 &63.39 &57.78 \\% %% In-table horizontal line % Summary/total row
%         \bottomrule % Bottom horizontal line
%         \end{tabular}}

%         \label{tab:results} 
%         \end{table*}% A label for referencing this table elsewhere, references are used in text as \ref{label}

% \newcommand{\resultstable}{% no arguments
% \begin{table}[!ht]
% \caption{Table captions should be placed above the}
%     \centering
%     \begin{tabular}{|l|l|l|l|l|}
%     \hline
%         \textbf{Models} & \textbf{Optimal Threshold } & \textbf{Accuracy} & \textbf{F1-Score}  & \textbf{AUCROC} \\ \hline
%         \multicolumn{5}{|l|}{\textbf{Imaging Model}} \\ \hline
%         PENet & 0.625 & 0.689 & 0.678 & 0.796 \\ \hline
        
%         \multicolumn{5}{|l|}{\textbf{EHR Models}} \\ \hline
%         ElasticNet & 0.59 & 0.837 & 0.85 & 0.913 \\ \hline
%         Normalising the whole dataset (1505 features) & 0.68 & 0.879 & 0.894 & 0.917 \\ \hline
%         Standardizing separately (1505 features) & 0.58 & 0.842 & 0.856 & 0.895 \\ \hline
%         Normalizing separately (1505 features) [a] & 0.68 & 0.879 & 0.894 & 0.917 \\ \hline
%         Standardisation before feature selection (finally 46) & 0.67 & 0.842 & 0.856 & 0.907 \\ \hline
%         Normalisation before feature selection (finally 46) & 0.73 & 0.874 & 0.89 & 0.909 \\ \hline
%         Standardisation after feature selection (finally 39) & 0.55 & 0.853 & 0.868 & 0.915 \\ \hline
%         Normalisation after feature selection (finally 39) [b] & 0.73 & 0.874 & 0.89 & 0.909 \\ \hline
        
%         \multicolumn{5}{|l|}{\textbf{Late Fusion}} \\ \hline
%         RadFusion & - & 0.89 & 0.902 & 0.946 \\ \hline
%         ElasticNet & 0.47 & 0.879 & 0.892 & 0.944 \\ \hline
%         Normalising the whole dataset (1505 features) & 0.46 & 0.889 & 0.905 & 0.948 \\ \hline
%         Standardizing separately (1505 features) & 0.47 & 0.879 & 0.892 & 0.94 \\ \hline
%         Normalizing separately (1505 features) [a] & 0.47 & 0.889 & 0.905 & 0.948 \\ \hline
%         Standardisation before feature selection (finally 46) & 0.47 & 0.868 & 0.882 & 0.94 \\ \hline
%         Normalisation before feature selection (finally 46) & 0.46 & 0.889 & 0.905 & 0.947 \\ \hline
%         Standardisation after feature selection (finally 39) & 0.47 & 0.874 & 0.889 & 0.949 \\ \hline
%         Normalisation after feature selection (finally 39) [b] & 0.46 & 0.884 & 0.901 & 0.945 \\ \hline
%     \end{tabular}
%     \label{table:results}
% \end{table}}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}





\begin{table}[]
\tiny
\caption{Ablation studies on (1) the inclusion of subsegmental cases in both training stages, (2) contrastive representation learning methods, (3) loss functions, and (4) pre-processing techniques}
\resizebox{1\linewidth}{!}{\begin{tabular}{ccccccccc}
\hline
\multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                         & \multicolumn{2}{c|}{Include Subsegmental}                                 & \multicolumn{1}{c|}{}                                                                               & \multicolumn{1}{c|}{}                                                                              & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                           &                              \\ \cline{3-4}
\multicolumn{1}{c|}{\multirow{-2}{*}{Exp. Set}} & \multicolumn{1}{c|}{\multirow{-2}{*}{Exp \#}} & \multicolumn{1}{c|}{Pre-training}   & \multicolumn{1}{c|}{Finetuning}     & \multicolumn{1}{c|}{\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Contrastive\\ Method\end{tabular}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Optimal\\ Threshold\end{tabular}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{Accuracy}} & \multicolumn{1}{c|}{\multirow{-2}{*}{F1 score}} & \multirow{-2}{*}{AUROC}      \\ \hline
                                                & 1.1                                           & {\color[HTML]{000000} $\checkmark$} & {\color[HTML]{000000} $\checkmark$} & InfoNCE                                                                                             & {\color[HTML]{000000} 36.17}                                                                       & {\color[HTML]{000000} 86.84}                    & {\color[HTML]{000000} 88.58}                    & {\color[HTML]{330001} 92.77} \\
                                                & 1.2                                           & {\color[HTML]{000000} $\checkmark$} & {\color[HTML]{000000} $\times$}     & InfoNCE                                                                                             & {\color[HTML]{000000} 35.31}                                                                       & {\color[HTML]{000000} 85.78}                    & {\color[HTML]{000000} 87.78}                    & {\color[HTML]{330001} 92.02} \\
                                                & 1.3                                           & {\color[HTML]{000000} $\times$}     & {\color[HTML]{000000} $\checkmark$} & InfoNCE                                                                                             & {\color[HTML]{000000} 38.07}                                                                       & {\color[HTML]{000000} 86.84}                    & {\color[HTML]{000000} 88.47}                    & {\color[HTML]{330001} 92.34} \\
\multirow{-4}{*}{1}                             & \textbf{1.4}                                           & {\color[HTML]{000000} \textbf{$\times$}}     & {\color[HTML]{000000} \textbf{$\times$}}     & \textbf{InfoNCE}                                                                                          & {\color[HTML]{000000} \textbf{39.36}}                                                                       & {\color[HTML]{000000} \textbf{88.94}}                  & {\color[HTML]{000000} \textbf{90.49}}                    & {\color[HTML]{330001} \textbf{94.03}} \\ \hline
                                                & 2.1                                           & {\color[HTML]{000000} $\times$}     & {\color[HTML]{000000} $\times$}     & SupCon                                                                                              & {\color[HTML]{000000} 39.80}                                                                       & {\color[HTML]{000000} 90.00}                    & {\color[HTML]{000000} 91.32}                    & {\color[HTML]{330001} 94.31} \\
\multirow{-2}{*}{2}                             & 2.2                                           & {\color[HTML]{000000} $\times$}     & {\color[HTML]{000000} $\times$}     & Barlow Twins                                                                                        & {\color[HTML]{000000} 48.75}                                                                       & {\color[HTML]{000000} 89.42}                    & {\color[HTML]{000000} 90.90}                    & {\color[HTML]{330001} 92.81} \\ \hline
                                                & 3.1                                           & $\times$                            & $\times$                            & SupCon                                                                                              & \multicolumn{1}{l}{}                                                                               & \multicolumn{1}{l}{}                            & \multicolumn{1}{l}{}                            & \multicolumn{1}{l}{}         \\
                                                & 3.2                                           & $\times$                            & $\times$                            & SupCon                                                                                              & \multicolumn{1}{l}{}                                                                               & \multicolumn{1}{l}{}                            & \multicolumn{1}{l}{}                            & \multicolumn{1}{l}{}         \\
\multirow{-3}{*}{3}                             & 3.3                                           & $\times$                            & $\times$                            & SupCon                                                                                              & \multicolumn{1}{l}{}                                                                               & \multicolumn{1}{l}{}                            & \multicolumn{1}{l}{}                            & \multicolumn{1}{l}{}         \\ \hline
\end{tabular}}
\end{table}

==> equations.tex <==
% adapted from \cite{infonce}, \cite{contrastivemedical}, is an image-EHR contrastive loss made up of two terms with the following expression:

\begin{equation}
    \label{eq:supcon}
\mathcal{L}_{PECon}=\sum_{i \in I} \frac{-1}{|P(i)|}\sum_{p \in P(i)} \frac{1}{2} \big(\ell^{c}_{i,p} + \ell^{e}_{i,p}\big)
\end{equation}
% where $D$ is the number of image-EHR pairs. The first term is an image-to-EHR loss, which can be expressed for the $i$-th pair as:
where $i \in I \equiv\{1...2D\} $ is the index of an arbitrary sample within a given batch used as the anchor feature, $P(i) \equiv \{p \in A(i): y_{p}=y_{i} \}$ is the set of indices of all samples within the batch having the same ground truth label as sample $i$ that are distinct from it, and $|P_{i}|$ is the set cardinality. The individual loss terms $\ell_{i,p}^{c}$ and $\ell_{i,p}^{e}$ can be expressed as:

\begin{equation}
    \label{eq:img-txt}
   \ell_{i,p}^{c} = log(\frac{exp{(\langle c_{i}.c_{p}\rangle \times \tau) }}{\sum_{a\in A(i)}exp{(\langle c_{i}.c_{a}\rangle \times \tau)}}) + log(\frac{exp{(\langle c_{i}.e_{p}\rangle \times \tau) }}{\sum_{a\in A(i)}exp{(\langle c_{i}.e_{a}\rangle \times \tau)}})
\end{equation}


\begin{equation}
    \label{eq:txt-img}
   \ell_{i,p}^{e} = log(\frac{exp{(\langle e_{i}.c_{p}\rangle \times \tau) }}{\sum_{a\in A(i)}exp{(\langle e_{i}.c_{a}\rangle \times \tau)}}) + log(\frac{exp{(\langle e_{i}.e_{p}\rangle \times \tau) }}{\sum_{a\in A(i)}exp{(\langle e_{i}.e_{a}\rangle \times \tau)}})
\end{equation}
where $\tau \in \mathcal{R}^{+}$ is a temperature parameter. This bi-directional objective aims to pull together the CT and EHR features corresponding to the same classes, while pushing apart the feature embeddings of opposite class, thereby maximising the agreement between same class and minimizing from the opposite class.
% corresponding image-EHR pairs while pulling apart representations from random pairings.
The visual  projection head $f_{c}$ and the EHR  projection head $f_{e}$ are then separately finetuned for classification by minimizing the cross-entropy loss. For this, the multimodal prediction is given by: 
% For final evaluation, we use late fusion of both models as follows:
\begin{equation}
    \label{eq:final-proba}
    \hat{y}_{x_{c},x_{e}}= \lambda \hat{y}_{x_{c}}+ (1-\lambda)\hat{y}_{x_{e}}
\end{equation}
where $\lambda$ is modality weighting scalar $\in [0,1]$, which can be used to set the influence each modality model will have on the overall multimodal classification. 

